FlexPool: A Distributed Model-Free Deep Reinforcement Learning Algorithm for Joint Passengers & Goods Transportation

The growth in online goods delivery is causing a dramatic surge in urban vehicle traffic from last-mile deliveries. On the other hand, ride-sharing has been on the rise with the success of ride-sharing platforms and increased research on using autonomous vehicle technologies for routing and matching. The future of urban mobility for passengers and goods relies on leveraging new methods that minimize operational costs and environmental footprints of transportation systems. This paper considers combining passenger transportation with goods delivery to improve vehicle-based transportation. Even though the problem has been studied with a defined dynamics model of the transportation system environment, this paper considers a model-free approach that has been demonstrated to be adaptable to new or erratic environment dynamics. We propose FlexPool, a distributed model-free deep reinforcement learning algorithm that jointly serves passengers & goods workloads by learning optimal dispatch policies from its interaction with the environment. The proposed algorithm pools passengers for a ride-sharing service and delivers goods using a multi-hop transit method. These flexibilities decrease the fleet's operational cost and environmental footprint while maintaining service levels for passengers and goods. Through simulations on a realistic multi-agent urban mobility platform, we demonstrate that FlexPool outperforms other model-free settings in serving the demands from passengers & goods. FlexPool achieves 30% higher fleet utilization and 35% higher fuel efficiency in comparison to (i) model-free approaches where vehicles transport a combination of passengers & goods without the use of multi-hop transit, and (ii) model-free approaches where vehicles exclusively transport either passengers or goods.

==> bio.tex <==
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{kaushik.jpg}}]{Kaushik Manchella} 
received the B.S. degree in Mechanical Engineering from Purdue University, West Lafayette, IN, USA in 2016. He is currently pursuing the M.S. degree in Industrial Engineering at Purdue University, West Lafayette, IN, USA. 

He has worked with consumer data services leveraging machine learning and AI to build new products. His research interests are in the areas of reinforcement learning, computer vision, and natural language processing.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{abhi.jpg}}]{Abhishek K. Umrawal}
received the M.Sc. degree in Statistics from the Indian Institute of Technology, Kanpur, India in 2011. He is currently pursuing the M.S. and Ph.D. degrees in Economics and Industrial Engineering at Purdue University, West Lafayette, IN, USA. 

His research interests include deep reinforcement learning, optimization, intelligent transportation, social networks, and computational economics.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{aggarwal.jpeg}}]{Vaneet Aggarwal (S'08 - M'11 - SM'15)}
received the B.Tech. degree from the Indian Institute of Technology, Kanpur, India in 2005, and the M.A. and Ph.D. degrees in 2007 and 2010, respectively from Princeton University, Princeton, NJ, USA, all in Electrical Engineering.
	
He is currently an Associate Professor at Purdue University, West Lafayette, IN, where he has been since Jan 2015. He was a Senior Member of Technical Staff Research at AT\&T Labs-Research, NJ (2010-2014), Adjunct Assistant Professor at Columbia University, NY (2013-2014), and VAJRA Adjunct Professor at IISc Bangalore (2018-2019). His current research interests are in communications and networking, cloud computing, and machine learning.
	
Dr. Aggarwal received Princeton University's Porter Ogden Jacobus Honorific Fellowship in 2009, the AT\&T Vice President Excellence Award in 2012, the AT\&T Key Contributor Award in 2013, the AT\&T Senior Vice President Excellence Award in 2014, the 2017 Jack Neubauer Memorial Award recognizing the Best Systems Paper published in the IEEE TRANSACTIONS ON VEHICULAR TECHNOLOGY, and the 2018 Infocom Workshop HotPOST Best Paper Award. He is on the Editorial Board of the IEEE TRANSACTIONS ON COMMUNICATIONS, the IEEE TRANSACTIONS ON GREEN COMMUNICATIONS AND NETWORKING, and the IEEE/ACM TRANSACTIONS ON NETWORKING.\end{IEEEbiography}


